Challenges in Quantitative Abstractions for Collective Adaptive Systems

Like with most large-scale systems, the evaluation of quantitative properties of collective adaptive systems is an important issue that crosscuts all its development stages, from design (in the case of engineered systems) to runtime monitoring and control. Unfortunately it is a difficult problem to tackle in general, due to the typically high computational cost involved in the analysis. This calls for the development of appropriate quantitative abstraction techniques that preserve most of the system's dynamical behaviour using a more compact representation. This paper focuses on models based on ordinary differential equations and reviews recent results where abstraction is achieved by aggregation of variables, reflecting on the shortcomings in the state of the art and setting out challenges for future research.

==> eptcsdata.tex <==
\providecommand{\firstpage}{62}
\providecommand{\publicationstatus}{M.H. ter Beek and M. Loreti (Eds.): Workshop on\\ 
FORmal methods for the quantitative Evaluation\\ 
of Collective Adaptive SysTems (FORECAST'16).\\
EPTCS 217, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.217.8}{10.4204/EPTCS.217.8}}
\pdfoutput=1

